LLM Support for Mathematical Problem Posing: What Changes When Revision Formulations Are Supplied or Withheld?

In mathematical problem posing, participants construct or modify problems rather than only solve predefined ones, creating opportunities for Large Language Models (LLMs) to support how those problems are formulated and revised. We investigate two forms of LLM support for revising participant-generated problems: Socratic scaffolding, which uses guiding questions while withholding candidate formulations, and Direct scaffolding, which provides concrete alternative formulations. We conducted a counterbalanced within-subjects study with 20 graduate students who posed and revised problems across two mathematical scenarios. Problems showed larger immediate supported artifact-quality gains under Direct than Socratic scaffolding. Exploratory dimension-level analyses identified statistically significant differences in structural clarity and novelty after correction for multiple comparisons. Socratic scaffolding was associated with longer revision time, highlighting a contrast between immediate artifact outcomes and revision processes. These findings identify the amount of candidate revision content supplied by an LLM as an important design variable in mathematical problem posing.

==> files/description.tex <==
\section{Discussion}
\label{sec:discussion}

This study compared two forms of LLM support for revising
participant-generated mathematical problems: Socratic scaffolding,
which provided guiding questions without a revised formulation, and
Direct scaffolding, which provided concrete alternative formulations.
This comparison is particularly relevant to problem posing because the
LLM is responding to a problem constructed by the participant and can
support the revision of that problem in different ways. We found larger
immediate problem-quality gains under Direct than Socratic scaffolding.
Exploratory dimension-level analyses showed statistically significant
condition differences after correction for structural clarity and
novelty, but not for conceptual accuracy and solvability or cognitive
demand. Secondary results showed higher pragmatic and overall
user-experience ratings under Direct scaffolding, whereas revision
intervals were longer under Socratic scaffolding. Together, these
findings show that the two forms of LLM revision support were associated
with different immediate artifact and interaction outcomes.

\subsection{Direct Produced Larger Quality Gains While Socratic Revisions Took Longer}

For RQ1, problems revised under Direct scaffolding showed larger
immediate quality gains than those revised under Socratic scaffolding.
One possible interpretation is that the concrete alternatives provided
under Direct scaffolding were more readily actionable during revision.
Participants could consider explicit formulations while deciding how to
revise their problems, whereas Socratic scaffolding provided questions
that still had to be interpreted and translated into a revision. This
interpretation is consistent with the user-experience results, in which
participants rated Direct scaffolding higher in pragmatic quality and
overall user experience.

The secondary behavioral results provide a different but complementary
view of the revision process. After accounting for task position,
revision intervals were approximately twice as long under Socratic
scaffolding. Illustrative interview accounts provide additional context
for this pattern. MC04 described Direct feedback as ``easier to act on''
while saying that Socratic feedback ``made me think more,'' and MC16
described Socratic feedback as ``asking questions to make me mentally
work,'' in contrast to Direct ``suggestions or specific ones.'' These
accounts illustrate how some participants experienced the two forms of
support, but they do not establish why Socratic revisions took longer or
that the longer revision intervals represented greater cognitive effort
or learning.

Considering the quality and process results together provides a more
complete picture than the quality difference alone. Direct scaffolding
was associated with larger immediate changes in the resulting problems
and was rated as more pragmatic, while Socratic scaffolding was
associated with longer revision intervals. The present data do not show
that one of these patterns is generally preferable to the other. Rather,
they indicate that different forms of LLM support can be associated with
both what is produced during revision and how the revision activity
proceeds.

This combination of findings can also be viewed through the assistance
dilemma, which concerns the balance between providing information and
leaving aspects of a task for the participant to work out
~\cite{KoedingerAleven2007Assistance}. Direct scaffolding made possible
revisions explicit, whereas Socratic scaffolding provided guidance
without specifying a revised formulation. Our findings do not resolve
this dilemma or identify an optimal level of assistance. Instead, they
show how two specific forms of assistance were associated with different
immediate artifact and revision-process outcomes when the object being
revised was a participant-generated mathematical problem.

These outcomes should also be interpreted within the distinction between
supported performance and learning
~\cite{SoderstromBjork2015LearningPerformance}. The larger quality gain
under Direct scaffolding reflects problems produced while LLM support
was available, whereas the longer Socratic revision interval does not by
itself indicate greater learning or cognitive engagement. Determining
whether either form of support produces different learning, retention,
or transfer would require subsequent unassisted measures. The
contribution of the present comparison is therefore more specific: it
examines two structured forms of LLM revision support within the same
study of participant-generated mathematical problems and evaluates their
immediate artifact and interaction outcomes.

\subsection{Condition Differences Were Evident for Clarity and Novelty}

For RQ2, the exploratory analyses showed statistically significant
Direct--Socratic differences after Holm correction for structural clarity
and novelty, but not for conceptual accuracy and solvability or cognitive
demand. These results help unpack the overall quality difference by
showing which individual rubric dimensions provided the clearest evidence
of a condition difference in this sample.

The structural-clarity result is consistent with the form of Direct
feedback. Providing complete alternative formulations gives participants
concrete examples of how a problem can be structured and expressed,
whereas Socratic feedback identifies aspects to reconsider through
questions without supplying a revised formulation. The larger clarity
gain under Direct scaffolding is therefore compatible with the greater
specificity of the support available during revision.

The novelty result is also notable. Direct feedback provided alternative
ways of formulating the participant's problem, which could expose
participants to problem framings that differed from their initial
versions. Problems revised under Direct scaffolding consequently showed
larger gains on the rubric's novelty dimension in this sample. This
finding concerns novelty as a property of the resulting artifact; it
should not be interpreted as evidence that participants themselves became
more original or creative.

In contrast, the adjusted analyses did not establish condition
differences for conceptual accuracy and solvability or cognitive demand.
A clearer or more novel formulation does not necessarily make a problem
more conceptually correct or cognitively demanding, so examining the
individual dimensions provides information that is not visible from the
aggregate quality score alone. At the same time, the dimension-specific
contrasts were not directly compared with one another. The different
patterns of statistical significance therefore should not be interpreted
as evidence that the condition effect was statistically larger for
clarity or novelty than for the other dimensions.

\subsection{Limitations and Future Directions}

This formative study involved 20 graduate computing students, two
mathematical scenarios, one LLM implementation, and two specific
scaffolding designs. The findings therefore need to be examined across
other populations, tasks, mathematical content, and LLM implementations.
The mathematical content was relatively elementary for this graduate
sample, and future studies should examine whether similar patterns occur
when participants pose and revise problems involving more demanding or
less familiar content. The two conditions also represent particular
implementations of Socratic and Direct support; the findings should not
be generalized to all question-based or direct scaffolding designs.

Several aspects of the design also limit what can be concluded from the
observed changes. The study did not include an unassisted revision
condition, so original-to-revised changes cannot isolate improvement
attributable specifically to LLM support from improvement associated with
revision, practice, or repeated engagement with the task. Repeated trials
also meant that later problems within a session were constructed after
participants had already received feedback under that condition, and
exposure to both conditions leaves open possible carryover despite
counterbalancing. In addition, feedback was generated dynamically by the
LLM, so individual feedback instances could vary within the same prompt
constraints.

Future work can address these limitations while examining how different
forms of support might be combined or adapted over time. Subsequent
unassisted tasks would help distinguish immediate supported artifact
quality from changes in independent problem-posing performance. Studies
with more demanding content and broader participant populations could
test the generality of the present findings. Scaffolding theory also
emphasizes contingent and fading support
~\cite{vanDePol2010Scaffolding}; accordingly, future studies could examine
adaptive or sequential designs in which question-based guidance and
concrete alternatives are introduced at different stages of revision
depending on participants' needs. Such work could move beyond comparing
two fixed forms of support toward understanding when different forms of
LLM assistance are useful during mathematical problem posing.

==> files/old_disc.tex <==
\section{Discussion}
\label{sec:discussion}


This study examined two forms of LLM support for revising
participant-generated mathematical problems: Socratic scaffolding, which
withheld candidate formulations and guided revision through questions, and
Direct scaffolding, which supplied alternative formulations. Direct scaffolding was associated with larger immediate overall
quality gains than Socratic scaffolding. %Exploratory dimension-level analyses provided the clearest evidence of condition differences for structural clarity and novelty. 
Together, the findings characterize how supplying versus withholding candidate revision formulations relates to both the resulting artifact and the revision process.


\subsection{Scaffolding Problems Rather Than Solutions}

Problem posing creates a distinct scaffolding setting because the
artifact being refined is a problem constructed by the participant rather
than a response to a predefined problem. The LLM can therefore respond to a participant-generated problem
while also supplying content that could become part of its revised form.
Our two designs instantiated this distinction by varying how much candidate
revision content the LLM supplied: Socratic scaffolding withheld candidate
formulations, whereas Direct scaffolding made possible revisions explicit.
This makes the amount of candidate formulation supplied by the system a
concrete design consideration for LLM-supported problem posing.


\subsection{How the Form of LLM Support Related to Immediate Revision}

For RQ1, immediate problem-quality gains were larger under Direct
than Socratic scaffolding. This difference does not establish a generally
preferable form of scaffolding. Rather, it shows how immediate artifact-quality change differed
between two implementations of LLM-supported revision: one that supplied
candidate formulations and one that withheld them.

This pattern can be interpreted through the assistance dilemma:
instructional systems must balance information giving with information
withholding rather than assuming that either is uniformly preferable
~\cite{KoedingerAleven2007Assistance}. In our setting, Direct scaffolding
made candidate revision content available, whereas Socratic scaffolding withheld candidate content and left participants to decide how, if at all, the guiding questions should be reflected in their revisions. Our findings place this established assistance dilemma in a
problem-posing setting where the assistance can include candidate
content for the artifact itself. The observed difference concerns
supported artifact quality and does not establish that greater assistance
is educationally preferable.

The larger immediate artifact gain under Direct scaffolding should
also be separated from claims about learning. The learning--performance
distinction emphasizes that performance observed while support is
available can be a poor indicator of durable changes in independent
capability~\cite{SoderstromBjork2015LearningPerformance}. Here, Direct
scaffolding supplied candidate formulations during the very activity whose
artifact was subsequently evaluated. A higher-quality supported problem
therefore establishes an immediate performance difference, but not that
participants acquired an equivalent ability to formulate revisions
independently. Establishing that claim would require subsequent unassisted
performance, retention, or transfer.


% NEW 2
The revision-time result provides a complementary process signal:
after accounting for task position, the recorded revision interval was
approximately twice as long under Socratic scaffolding. This measure
captures revision after feedback inspection rather than total interaction
time. Participant accounts help contextualize
this difference. MC04 described Direct feedback as ``easier to act on''
while saying Socratic feedback ``made me think more,'' and MC16 described
Socratic feedback as ``asking questions to make me mentally work,'' in
contrast to Direct ``suggestions or specific ones.'' These accounts are
consistent with the design distinction between making candidate content
available and leaving participants to determine how guidance should be
translated into revision. They do not, however, establish that the longer
revision time represented greater cognitive effort or learning.


\subsection{Exploratory Differences Across Quality Dimensions}
Problem-posing quality is commonly evaluated through multiple
properties of the posed problem rather than through a single
characteristic~\cite{cai2013mathematical,cai2023impact,
Silber2021ProblemPosing}. Consistent with this view, our rubric separately
represented conceptual accuracy and solvability, structural clarity,
cognitive demand, and novelty. The exploratory analyses for RQ2 therefore
examined these dimensions separately in addition to the aggregate quality
score.

The exploratory analyses for RQ2 provide a more detailed view of
the overall condition difference. After correction for multiple comparisons, evidence of a
Direct--Socratic difference was clearest for structural clarity and
novelty, whereas evidence for conceptual accuracy and cognitive demand
was more uncertain. These analyses tested each dimension-specific
contrast rather than whether the condition effects differed from one
dimension to another.


These dimensions describe different properties of a posed
problem. A problem may, for example, be clearly formulated without
necessarily requiring greater reasoning, while a cognitively demanding
problem may still contain ambiguity. Reporting dimension-level estimates
alongside the aggregate score therefore provides additional descriptive
information about the revised artifacts. Novelty therefore describes a property of the revised artifact, not greater participant-generated originality.


\subsection{Implications for LLM-Supported Problem Posing}

Taken together, the findings identify the amount of candidate
revision content supplied by an LLM as an important design consideration
for LLM-supported problem posing. In this study, supplying explicit
alternatives was associated with larger immediate artifact-quality gains
than withholding them. This comparison does not establish a generally
preferable scaffolding strategy, but it shows why the form of assistance
should be made explicit when designing and evaluating LLM-supported
revision.


The findings also have implications for how such systems are
evaluated. Immediate artifact quality and independent participant
capability are distinct evaluation targets. A system can contribute to a
higher-quality posed problem without establishing that the participant has
acquired the ability to produce the same improvement independently.
Accordingly, evaluations aimed at learning should complement artifact-level
outcomes with independent measures of subsequent performance, retention,
or transfer.




% OLD 2
% [Current Limitations and Future Work subsection]

% NEW 2
\subsection{Limitations and Future Directions}
This formative study involved 20 graduate computing students,
two mathematical scenarios, one LLM implementation, and two specific
feedback designs, so broader evaluation across populations, tasks, and
LLM implementations is needed. Because there was no unassisted revision
condition, the observed artifact changes do not establish independently
acquired improvement. In addition, repeated trials and exposure to both
conditions leave open possible carryover to later problem construction,
despite counterbalancing. The mathematical content was also relatively elementary for this
graduate sample; future work should examine whether the observed patterns
hold when participants revise problems involving more demanding or
less familiar content.

Future work can examine unassisted performance and adaptive forms
of support. Scaffolding theory's emphasis on contingent and fading
support~\cite{vanDePol2010Scaffolding} motivates testing when candidate
formulations should be supplied or withheld rather than keeping support
fixed throughout a session.
